Single Loop Gaussian Homotopy Method for Non-convex Optimization

The Gaussian homotopy (GH) method is a popular approach to finding better stationary points for non-convex optimization problems by gradually reducing a parameter value $t$, which changes the problem to be solved from an almost convex one to the original target one. Existing GH-based methods repeatedly call an iterative optimization solver to find a stationary point every time $t$ is updated, which incurs high computational costs. We propose a novel single loop framework for GH methods (SLGH) that updates the parameter $t$ and the optimization decision variables at the same. Computational complexity analysis is performed on the SLGH algorithm under various situations: either a gradient or gradient-free oracle of a GH function can be obtained for both deterministic and stochastic settings. The convergence rate of SLGH with a tuned hyperparameter becomes consistent with the convergence rate of gradient descent, even though the problem to be solved is gradually changed due to $t$. In numerical experiments, our SLGH algorithms show faster convergence than an existing double loop GH method while outperforming gradient descent-based methods in terms of finding a better solution.

==> 5_ZOSLGHerror.tex <==
\section{Zeroth-order single loop Gaussian homotopy algorithm with error tolerance}
\label{sec:error}
In the previous sections, we assumed that we had access to the exact function value or a gradient oracle whose variance was finite. However, in some practical cases, we will have access only to the function values containing error, and it would be impossible to obtain accurate gradient oracles of an underlying objective function. Figure \ref{fig:smooth_and_error} illustrates such a case; although the objective function $f$ (Figure \ref{fig:smooth}) is smooth, the accessible function $f'$ (Figure \ref{fig:error}) contains some error, and thus many local minima arise. In this section, we consider optimizing a smooth objective function $f$ using only the information of $f'$. We assume that the following condition holds between $f$ and $f'$.

\begin{figure}
\centering
\begin{tabular}{lc}
    %\hspace{-5mm}
    \subfigure[Smooth objective function]{
    \label{fig:smooth}
    \begin{minipage}[t]{0.50\linewidth}
        \centering
        \includegraphics[width=1.5in]{images_new/func_smooth.png}
        \vspace{1mm}
    \end{minipage}%
    }
    \subfigure[Accessible function with error]{
    \label{fig:error}
    \begin{minipage}[t]{0.50\linewidth}
        \centering
        \includegraphics[width=1.5in]{images_new/func_with_error.png}
        \vspace{1mm}
     \end{minipage}
    }
\end{tabular}
\centering
\caption{Illustration of a smooth objective function and the  accessible function that contains error.}
\label{fig:smooth_and_error}
\end{figure}

\begin{assumption}{A3}\label{A3}$\ $
\renewcommand{\labelenumi}{(\roman{enumi})}
The supremum norm of the difference between $f$ and $f'$ is uniformly bounded:
$$\sup_{x\in\mathbb{R}^d}|f(x)-f'(x)|\leq\nu.$$
In the stochastic setting, we assume $\sup_{x\in\mathbb{R}^d}|f(x;\xi)-f'(x;\xi)|\leq\nu$ for any $\xi$.
\end{assumption}
Please note that we do not impose any other assumptions on the accessible function $f'$. Thus, $f'$ can be non-Lipschitz or even discontinuous. Even in such cases, we can develop an algorithm with a convergence guarantee because its smoothed function $F'(x,t)$ is smooth as far as $t$ is sufficiently large. In the following, we denote the Lipschitz and gradient Lipschitz constant of $F'(\cdot,t)$ as $L_0(t)$ and $L_1(t)$, respectively. 

The ZOSLGH algorithm in this setting is almost the same as Algorithm \ref{alg:ZOGH}. The only difference is $\sqrt{\nu}$ rather than $\epsilon$ in the update rule of $t_{k+1}$. See the Algorithm \ref{alg:ZOGH_error} in the Appendix for a more detailed description.

We provide the convergence analysis only for the deterministic setting in the following theorem.
The proof and the definition of $\hat{x}$ are given in Appendix~\ref{subsec:proof_error_deterministic}.
For the stochastic setting, see Appendix \ref{subsec:proof_error_stochastic}.
\begin{theorem}[\textbf{Convergence of ZOSLGH with error tolerance, Deterministic setting}]
    \label{thm:error_deterministic}
    Suppose Assumptions~\ref{A1} and \ref{A3} hold, and set the stepsize for $x$ at iteration $k$ as $\beta_k=\frac{1}{16(d+4)L_1(t_k)}\ ,k\in[T]$.
    % If the error level $\nu$ satisfies $\nu=O(t_k^2)\ (k\in[T])$, the output sequence of the ZOSLGH algorithm $\{x_k\}_{k=1}^T$ will then satisfy 
    % $
    %     \frac{1}{T}\sum_{k=1}^T \mathbb{E}[\|\nabla f(x_k)\|^2]
    %     = O\left(\frac{d}{T}\left(1+\sqrt{d}\sum_{k=1}^T\mathbb{E}_u[|t_{k+1}-t_k|] + d^2\sum_{k=1}^T\mathbb{E}_u[t_k^2]\right)\right)
    % $,
    % where the expectation is taken w.r.t.~random vectors $\{u_k\}$.
    % Consequently,
    % if we update $t_k$ as in Algorithm~\ref{alg:ZOGH_error} with an arbitrary constant $\gamma \in (0, 1)$,
    Then,
    for any setting of the parameter $\gamma$,
    if the error level $\nu$ satisfies $\nu=O(\epsilon^2/d^3)$,
    we can find $\hat{x}$ satisfying
    $\mathbb{E}[ \|\nabla f(\hat{x})\| ] \leq\epsilon$ with the iteration complexity of 
    $T = O({d^{3}}/{\epsilon^2})$,
    where the expectation is taken w.r.t.~random vectors $\{u_k\}$ and $\{v_k\}$.
    Further,
    if we choose $\gamma \leq d^{-\Omega(\epsilon^2 / d)}$,
    the iteration complexity can be bounded as
    $T = O({d}/{\epsilon^2})$.
\end{theorem}

%This theorem indicates that we can reach an $\epsilon$-stationary point in $O(d^{3+\alpha}/\epsilon^2)$ iterations if the error level $\nu$ satisfies $\nu=O(\epsilon^2/d^{3-\alpha}),\ 0\leq\alpha\leq 3$. \memo{SI}{Does this follow from the above theorem?}
%================================================================================================%

